Multilingual analysis of intelligibility classification using English, Korean, and Tamil dysarthric speech datasets

This paper analyzes dysarthric speech datasets from three languages with different prosodic systems: English, Korean, and Tamil. We inspect 39 acoustic measurements which reflect three speech dimensions including voice quality, pronunciation, and prosody. As multilingual analysis, examination on the mean values of acoustic measurements by intelligibility levels is conducted. Further, automatic intelligibility classification is performed to scrutinize the optimal feature set by languages. Analyses suggest pronunciation features, such as Percentage of Correct Consonants, Percentage of Correct Vowels, and Percentage of Correct Phonemes to be language-independent measurements. Voice quality and prosody features, however, generally present different aspects by languages. Experimental results additionally show that different speech dimension play a greater role for different languages: prosody for English, pronunciation for Korean, both prosody and pronunciation for Tamil. This paper contributes to speech pathology in that it differentiates between language-independent and language-dependent measurements in intelligibility classification for English, Korean, and Tamil dysarthric speech.

==> figures/analysis.tex <==
\begin{figure}[t] %%% t: top, b: bottom, h: here
\centering
\caption{
Comparison of the languages with more than $10\%$ (Green) and less than $1\%$ (Red) CER improvements over the corresponding fine-tuning baseline.
}
\includegraphics[width=0.45\textwidth]{figures/analysis_pdf.pdf}
\label{fig:analysis}
\end{figure}

==> figures/features_tbl.tex <==
\begin{table*}[]
\caption{Acoustic measurements}
\vspace{2mm}
\label{tab:features}
\centering

% \resizebox{0.8\textwidth}{!}{

\begin{tabular}{c|c|c}

\hline
\multicolumn{2}{c|}{Category} & Features \\

\hline
\multicolumn{2}{c|}{Voice quality} & jitter, shimmer, PPQ, APQ, HNR, number of voice breaks, degree of voice breaks \\
\hline

% \hline
% \multirow{2}{*}{Voice quality} & Glottal flow & jitter, shimmer, PPQ, APQ, HNR \\
% \cline{2-3}
% & Phonation & \# of voice breaks, \% of voice breaks \\
% \hline

\multirow{2}{*}{Pronunciation} & Phoneme correctness & PCC, PCV, PCP \\
\cline{2-3}
& Vowel distortion & triangular VSA, quadrilateral VSA, FCR, VAI, F2-Ratio \\
\hline

\multirow{5}{*}{Prosody} 
& Speech rate & speaking rate, articulation rate, number of pauses, pause duration, phone ratio \\
\cline{2-3}
& Pitch & mean, median, std, min, max, range of F0 \\
\cline{2-3}
& Intensity & mean, median, std, min, max, range of energy \\
\cline{2-3}
& Rhythm & \%V, deltaV/C, VarcoV/C, rPVIV/C, nPVIV/C \\
\cline{2-3}
\hline

\end{tabular}
% }
\end{table*}

==> figures/features_tbl_old.tex <==
\begin{table*}[]
\caption{Acoustic measurements}
\vspace{2mm}
% \label{tab:features}
\centering

% \resizebox{0.8\textwidth}{!}{

\begin{tabular}{c|c|c}

\hline
\multicolumn{2}{c|}{Category} & Features \\

\hline
\multicolumn{2}{c|}{\multirow{2}{*}{Voice quality}} & jitter, shimmer, PPQ, APQ, HNR, \\
\multicolumn{2}{c|}{} & \# of voice breaks, \% of voice breaks \\
\hline
\multirow{2}{*}{Pronunciation} & Phoneme Correctness & PCC, PCV, PTC \\
\cline{2-3}
& Vowel distortion & triangular VSA, quadrilateral VSA, FCR, VAI, F2-Ratio \\
\hline

\multirow{5}{*}{Prosody} 
& \multirow{2}{*}{Speech rate} & speech duration, total duration, \\
& & speaking rate, articulation rate \\
\cline{2-3}
& Pitch & mean, median, std, min, max of F0 \\
\cline{2-3}
& Intensity & mean, range of energy \\
\cline{2-3}
& rhythm & \%V, deltaV/C, VarcoV/C, rPVIV/C, nPVIV/C \\
\cline{2-3}
\hline

\end{tabular}
% }
\end{table*}

==> figures/praat_tbl.tex <==
\begin{table}[h]
\caption{
Praat settings
}
\label{tab:praat}
% \vspace{-2mm}
%\scriptsize
\centering
%\resizebox{0.\textwidth}{!}{
\begin{tabular}{c|c}
\hline
Variables & Values (Hz) \\
\hline
minimum pitch & 50  \\
maximum pitch & 625  \\
pitch silence threshold & 0.03 \\
pitch voicing threshold & 0.45 \\
pitch octave cost & 0.01 \\
pitch octave jump cost & 0.35 \\
pitch voiced unvoiced cost & 0.14 \\
\hline
\end{tabular}
%}
\end{table}



==> figures/stats_tbl.tex <==
\begin{table*}[t]
\caption{Mean values of measurements}
\label{tab:analysis2}
\centering
\resizebox{0.9\textwidth}{!}{

\begin{tabular}{cc|c|c|c|c|c|c|c|c|c|c|c|c|c}

\hline
\multicolumn{2}{c|}{\multirow{2}{*}{Measurements}} & \multicolumn{4}{c|}{English} & \multicolumn{4}{c|}{Korean} & \multicolumn{4}{c}{Tamil} \\
\cline{3-14}
& & healthy & mild & moderate & severe & healthy & mild & moderate & severe & healthy & mild & moderate & severe \\
\cline{1-14}
\multirow{7}{*}{Voice quality} & jitter & 2.31 & 2.37 & 1.64 & 2.79 & 1.72 & 1.59 & 1.95 & 1.88 & 1.47 & 1.23 & 1.18 & 1.37\\
& shimmer & 12.07 & 9.97 & 5.97 & 9.46 & 7.53 & 6.91 & 8.28 & 7.29 & 8.07 & 7.15 & 7.00 & 7.57\\
& PPQ & 1.11 & 1.14 & 0.70 & 1.52 & 0.78 & 0.68 & 0.86 & 0.83 & 0.68 & 0.60 & 0.54 & 0.73\\
& APQ & 6.94 & 5.63 & 2.85 & 5.21 & 3.25 & 3.16 & 3.99 & 3.21 & 3.64 & 3.39 & 3.34 & 4.14\\
& HNR & 9.95 & 11.39 & 18.03 & 11.96  & 16.27 & 16.82 & 15.80 & 16.31 & 14.01 & 15.72 & 15.67 & 15.26\\
& number of VBs & 6.83 & 6.86 & 9.85 & 12.84 & 6.51 & 9.47 & 11.06 & 14.36 & 4.05 & 3.73 & 3.81 & 3.61\\
& degree of VBs & 16.49 & 19.04 & 25.94 & 23.33 & 1.72 & 1.59 & 1.95 & 1.88 & 19.93  & 18.26 & 20.79 & 19.64 \\
\cline{1-14}
\multirow{8}{*}{Pronunciation} & PCC & 95.93 & 94.25 & 71.08 & 59.76 & 97.53 & 83.47 & 50.92 & 12.18 & 93.17 & 70.42 & 53.08 & 26.90 \\
& PCV & 95.93 & 94.25 & 71.08 & 59.76 & 99.04 & 88.90 & 65.96 & 25.34 & 91.52 & 65.90 & 50.16 & 29.35 \\
& PCP & 95.28 & 93.79 & 67.93 & 57.35 & 98.20 & 85.85 & 57.48 & 17.90 & 92.63 & 69.08 & 52.28 & 27.68 \\
\cline{2-14}
& triangular VSA & 109791 & 110459 & 50541 & 60574 & 199831 & 149994 & 97226 & 62400 & 207104 & 97715 & 85328 &35626 \\
& quadrilateral VSA & 162175 & 169389 & 102766 & 74430 & 202496 & 149031 & 95282 & 67779 & 240516 & 114907 & 97589 & 42085 \\
& FCR & 1.28 & 1.25 & 1.38 & 1.46 & 1.35 & 1.40 & 1.67 & 1.85 & 1.54 & 1.37 & 1.47 & 1.64\\
& VAI & 0.80 & 0.81 & 0.73 & 0.69 & 0.78 & 0.75 & 0.63 & 0.55 & 0.89 & 0.74 & 0.70 & 0.63 \\
& F2-Ratio & 1.36 & 1.43 & 1.31 & 1.29 & 1.56 & 1.55 & 1.25 & 1.12 & 2.13 & 1.67 & 1.53 & 1.31\\
\cline{1-14}
\multirow{25}{*}{Prosody} & speaking rate & 2.96 & 2.80 & 2.49 & 2.90 & 3.41 & 2.79 & 2.33 & 1.59 & 2.49 & 0.72 & 2.43 & 2.62\\
& articulation rate & 6.39 & 6.11 & 4.78 & 5.57 & 5.67 & 5.20 & 5.33 & 5.74 & 5.46 & 4.57 & 4.31 & 4.04\\
& number of pauses & 1.40 & 1.65 & 4.90 & 3.80 & 1.49 & 3.49 & 5.73 & 8.13 & 2.14 & 2.25 & 2.31 & 2.48 \\
& pause duration & 2.44 & 2.58 & 4.18 & 3.87 & 1.52 & 2.93 & 5.00 & 10.90 & 1.85 & 1.37 & 1.47 & 1.11 \\
& phone ratio & 0.46 & 0.46 & 0.52 & 0.52 & 0.60 & 0.54 & 0.45 & 0.32 & 0.46 & 0.69 & 0.57 & 0.66\\
\cline{2-14}
& F0 mean & 60.03 & 69.53 & 87.45 & 93.21 & 98.57 & 91.55 & 80.91 & 74.39 & 88.44 & 110.04 & 124.31 & 148.94\\
& F0 median & 158.57 & 185.68 & 166.09 & 155.01 & 188.18 & 191.71 & 188.77 & 227.05 & 294.13 & 193.03 & 230.86 & 234.81\\
& F0 std & 90.10 & 96.06 & 90.70 & 95.43 & 95.64 & 97.76 & 99.29 & 109.38 & 106.23 & 95.52 & 114.46 & 112.01\\
& F0 min & 106.53 & 112.40 & 91.98 & 87.94 & 102.17 & 103.20 & 102.50 & 97.36 & 149.14 & 141.44 & 157.15 & 153.33\\
& F0 max & 420.77 & 394.67 & 401.32 & 449.69 & 261.97 & 339.47 & 436.04 & 450.51 & 311.67 & 258.36 & 307.79 & 285.48\\
& F0 range & 314.23 & 282.27 & 309.35 & 361.75 & 159.80 & 236.27 & 333.54 & 353.15 & 162.53 & 116.92 & 150.64 & 132.15\\
\cline{2-14}
& energy mean & 53.02 & 56.36 & 57.50 & 63.24 & 51.64 & 49.52 & 48.35 & 45.46 & 40.21 & 42.03 & 40.68 & 48.45\\
& energy median & 49.29 & 51.22 & 58.56 & 62.10 & 58.98 & 53.21 & 48.80 & 43.98 & 39.93 & 46.92 & 44.72 & 55.10\\
& energy std & 12.26 & 13.19 & 15.96 & 14.10 & 19.34 & 17.48 & 15.64 & 15.45 & 22.07 & 17.57 & 17.91 & 17.40\\
& energy min & 39.92 & 41.56 & 34.25 & 43.50 & 15.17 & 15.89 & 17.16 & 15.97 & 12.63 & 12.48 & 11.98 & 13.42\\
& energy max & 77.50 & 81.96 & 82.95 & 86.84 & 77.24 & 75.84 & 77.10 & 80.36 & 73.76 & 0 & 66.45 & 66.29 & 70.57\\
% & energy range & 37.58 & 40.41 & 48.70 & 43.34 & 62.07 & 59.95 & 59.94 & 64.39 & 61.14 & 53.97 & 54.30 & 57.15\\
\cline{2-14}
& \%V & 41.72 & 41.45 & 45.65 & 46.18 & 84.07 & 85.91 & 87.70 & 91.18 & 47.09 & 54.78 & 54.28 & 59.68\\
& deltaV & 60.70 & 63.19 & 131.37 & 124.19 & 475.79 & 787.42 & 1153.54 & 2971.46 & 62.06 & 71.92 & 76.44 & 87.18\\
& deltaC & 73.28 & 73.72 & 133.00 & 151.02 & 53.38 & 103.58 & 153.93 & 280.42 & 59.79 & 65.60 & 69.65 & 59.37\\
& VarcoV & 53.18 & 52.66 & 48.02 & 49.52 & 90.88 & 90.45 & 92.84 & 121.45 & 52.51 & 47.64 & 54.26 & 53.02\\
& VarcoC & 50.89 & 49.86 & 57.54 & 62.76 & 45.04 & 60.47 & 78.29 & 117.91 & 530.55 & 54.30 & 61.05 & 56.71\\
& rPVIV & 66.20 & 67.47 & 145.11 & 139.97 & 454.49 & 758.96 & 1083.72 & 2324.55 & 73.08 & 81.13 & 87.78 & 99.35\\
& rPVIC & 81.85 & 77.76 & 141.92 & 170.44 & 66.88 & 120.21 & 179.87 & 321.56 & 72.74 & 78.69 & 83.05 & 71.09\\
& nPVIV & 55.85 & 55.22 & 52.42 & 52.79 & 84.37 & 86.47 & 92.23 & 105.95 & 60.27 & 52.27 & 61.48 & 61.00 \\
& nPVIC & 56.89 & 53.14 & 63.30 & 65.06 & 53.44 & 55.58 & 82.73 & 107.32 & 59.81 & 62.57 & 69.52 & 65.52\\

\hline

\end{tabular} 
}
\end{table*}

